Winning the NIST Contest: A scalable and general approach to differentially private synthetic data

We propose a general approach for differentially private synthetic data generation, that consists of three steps: (1) select a collection of low-dimensional marginals, (2) measure those marginals with a noise addition mechanism, and (3) generate synthetic data that preserves the measured marginals well. Central to this approach is Private-PGM, a post-processing method that is used to estimate a high-dimensional data distribution from noisy measurements of its marginals. We present two mechanisms, NIST-MST and MST, that are instances of this general approach. NIST-MST was the winning mechanism in the 2018 NIST differential privacy synthetic data competition, and MST is a new mechanism that can work in more general settings, while still performing comparably to NIST-MST. We believe our general approach should be of broad interest, and can be adopted in future mechanisms for synthetic data generation.

==> ack.tex <==
%!TEX root = paper.tex
\vspace{1ex}
{\footnotesize
\noindent\textbf{Acknowledgements:}  This work was supported by the National Science Foundation under grants 1253327, 1408982, 1409125, 1443014, 1421325, and 1409143; and by DARPA and SPAWAR under contract N66001-15-C-4067. The U.S. Government is authorized to reproduce and distribute reprints for Governmental purposes not withstanding any copyright notation thereon. The views, opinions, and/or findings expressed are those of the author(s) and should not be interpreted as representing the official views or policies of the Department of Defense or the U.S. Government. \par
}


==> alg_outline.tex <==
\gm{Here is an attempt at a more detailed algorithm description.}


\begin{outline}[enumerate]
\1 {\bf Noise calibration}
\2[-] Input: target $\epsilon, \delta$ values
\2[-] Output: noise magnitude $\sigma$ used in Gaussian Mechanism invocations.

\1 {\bf Data transformation}
\2[-] Input: Original dataset $D_0$
\2[-] Output: Transformed dataset $D_1$

\1 {\bf Data-dependent domain compression}
\2 {\bf Measurement}: all one-way marginals
  \3[-] Input: $D_1, \sigma$
  \3[-] Output: $l_1 \leftarrow$ [new measurement log records]

\2 {\bf Thresholding}
  \3[-] Input: $l_1$
  \3[-] Output: [new dataset or new domain?]

\1 {\bf Measurement selection}
  \2[-] Input: provisional dataset
  \2[-] Output: $M \leftarrow$ selected 2-way and 3-way marginals

\1 {\bf Measurement}
  \2[-] Input: $D_1, M, \sigma$
  \2[-] Output: $l_2 \leftarrow$ [new measurement log records]

\1 {\bf Inference}
  \2[-] Input: measurements $l_1 \cup l_2$
  \2[-] Output: $P_\theta \leftarrow$ {\tt PGM.estimate}$(l_1 \cup l_2)$

\1 {\bf Synthetic data generation}
  \2[-] Input: $P_\theta$
  \2[-] Output: $D_2$

\1 {\bf Inverse data transformation}
  \2[-] Input: $D_2$
  \2[-] Output: $D_3$
\end{outline}



==> experiments_old.tex <==
\section{Experiments}

\begin{table}[t]
    \def\arraystretch{1.1}
    \centering\small
    \begin{tabular}{cc|ccc|c}
  \hline
  $\epsilon$ & Team & Metric \#1 & Metric \#2 & Metric \#3 & Overall \\ \hline
  0.3 & RMcKenna (\mech) & \textbf{0.17} & \textbf{0.12} & 0.10 & \textbf{0.13} \\
  0.3 & DPSyn & 0.31 & 0.15 & \textbf{0.07} & 0.18 \\
  \rowcolor{blue!10} 0.3 & \texttt{MST} & \textbf{0.13} & 0.18 & 0.22 & 0.18 \\
  0.3 & PrivBayes & 0.19 & 0.29 & 0.18 & 0.22 \\
  0.3 & Gardn999 & 0.32 & 0.21 & 0.25 & 0.26 \\
  0.3 & UCLANESL & 0.72 & 0.57 & 0.22 & 0.50 \\
  \hline
  1.0 & RMcKenna (\mech) & \textbf{0.15} & \textbf{0.09} & \textbf{0.04} & \textbf{0.09} \\
  1.0 & DPSyn & 0.23 & 0.11 & 0.05 & 0.13 \\
  \rowcolor{blue!10} 1.0 & \texttt{MST} & \textbf{0.09} & 0.16 & 0.20 & 0.15 \\
  1.0 & PrivBayes & 0.17 & 0.26 & 0.09 & 0.17 \\
  1.0 & Gardn999 & 0.28 & 0.18 & 0.22 & 0.23 \\
  1.0 & UCLANESL & 0.53 &0.42 & 0.28 & 0.41 \\
  \hline
  8.0 & RMcKenna (\mech) & 0.14 & \textbf{0.07} & 0.04 & \textbf{0.08} \\
  8.0 & DPSyn & 0.20 & 0.09 & \textbf{0.02} & 0.10 \\
  \rowcolor{blue!10} 8.0 & \texttt{MST} & \textbf{0.08} & 0.14 & 0.22 & 0.15\\
  8.0 & PrivBayes & \textbf{0.13} & 0.23 & 0.09 & 0.15 \\
  8.0 & Gardn999 & 0.26 & 0.17& 0.24 & 0.22\\
  8.0 & UCLANESL & 0.41 & 0.35 & 0.25 & 0.34 \\
  \hline
\end{tabular}
\caption{\label{table:experiments} Evaluation of \mech and other mechanisms from competing teams, broken down by the three scoring metrics: 3-way marginals, high-order conjunctions, and income inequality.  \texttt{MST} is also shown for comparison, even though that mechanism was not submitted during the competition.  If it was used, it would have placed third overall, but first on the 3-way marginal metric.}
\end{table}



In this section we discuss the experimental evaluation carried out by the contest organizers, and how \mech compared to the submissions from other teams.  We offer our own insights into the numbers and explanations fo rthe differences between mechansisms.

Evaluations were carried out on census data for two different states, Arizona and Vermont.  These datasets had \num{293999} and \num{211228} records, respectively.  Scores were calculated separately for each of the three evaluation metrics described in \cref{sec:eval}.  The final score was calculated by averaging the scores for each evaluation metric, each value of $\epsilon$, and each of the two datasets.  In \cref{table:experiments} we show the score breakdown by metric (averaged over Arizona and Vermont) for the top five submitted algorithms.  We also evaluted \texttt{MST} and included that as an extra row, even though it was not evaluating by the contest organizers at the time of the competition.

\mech consistently performed the best across the board, for most metrics and values of $\epsilon$.  Compared to DPSyn, it did a much better job at answering 3-way marginals, but slightly worse at handling the income inequality metric.   Compared to PrivBayes, \mech did slightly better on 3-way marginals, and much better on the other two metrics.  

These results confirm the merits of measuring overlapping marginals, as \mech and PrivBayes do, since these  mechanisms performed the best on the 3-way marginal metric.  DPSyn and Gardn999 clustered attributes into disjoint groups for measurement, losing information about the correlation between groups, and their scores on the 3-way marginal metric suffered as a result.

Generally speaking, \mech and DPSyn seemed to be the only mechanisms that scored well on the income inequality metric, which is surprising given that it was the simplest metric and only required preserving one 3-way marginal accurately.  This raises an important point: mechanisms that understood the evaluation criteria well, and designed their mechanisms around it, generally performed better than mechanisms that just tried to generate good synthetic data without thinking about how it's utility would be evaluated.  \mech and DPSyn did a good job of designing their mechanism for the task at hand, which was an important contributing factor for why they outperformed the other solutions.

While \mech relied heavily on the provisional dataset for measurement selection, the more general variant \texttt{MST} still performed well, without explicitly relying on the provisional data.  In would have won third place if it was submitted during the time of the competition.  As seen in \cref{table:experiments}, \texttt{MST} performed better than every other mechanism on the 3-way marginal metric.  Performance suffered on the income inequality metric, but this is not surprising because it is a general-purpose mechanism that doesn't explicitly try to presreve the required 3-way marginal for that metric.  This could also explain why it actually did better than \mech on the 3-way marginal metric: \mech allocate a significant weight to the $\marginal{SEX,CITY,\INCWAGEA}$ marginal, but this reduced the weight assigned to other measured marginals.   \texttt{MST} did not measure this marginal, so it could give more weight to the other measured marginals, which could explain why it did better on the 3-way marginal metric.  The fact that \texttt{MST} performed so well is pretty remarkable, given that it allocated one third of the privacy budget for measurement selection, and two thirds of the privacy budget for taking the measurements via the Gaussian mechanism.  Thus, while provisional data is certainly useful for measurement selection and algorithm design more generally, it is not necessary to generate high quality synthetic data.

For a much more comprehensive evaluation of these mechanisms, we refer the reader to the work of Bowen and Snoke \cite{bowen2019comparative}, which goes well beyond the metrics used in the competition to evaluate the mechanisms.  This work is also a useful resource that summarizes each mechanism at a high level.  The results in this paper generally show that \mech was the best performing mechanism for many of the additional evaluation metrics not used as part of the official scoring criteria.  This suggest that \mech produces the most generally useful synthetic data among the submitted mechanisms.  


==> graphical_models.tex <==
\section{Graphical Models}

\paragraph*{\textbf{Marginals}}
When dealing with high-dimensional data, it is common to work with {\em marginals} defined over a subset of attributes.  Let $C \subseteq [d]$ identify a subset of attributes and, for $\x \in \X$, let $\x_C = (x_i)_{i \in C}$ be the sub-vector of $\x$ restricted to $C$. Then the marginal vector (or simply ``marginal on C'') $\bmu_C$, is defined by:
%
$$ \bmu_C(\x_C) = \sum_{i=1}^m \I\{ \x^{(i)}_C = \x_C\}, \quad \forall \x_C \in \dom_C := \prod_{i \in C} \dom_i. $$
%
The size of the marginal is  $n_C := |\dom_C| = \prod_{i \in C} n_i$, which is exponential in $|C|$ but may be considerably smaller than $n$.

\begin{example}[Marginals] \label{example:marginals}
The $(gender, city)$ and $(gender, party)$ marginals are shown for the registered voters dataset introduced in \cref{example:toydata}.

\begin{table*}[h]
\captionsetup[subtable]{position = below}
\captionsetup[table]{position=top}
\begin{subtable}{0.22\textwidth}
\begin{tabular}{cc|c}
\multicolumn{2}{c}{$\x_{12}$} & $\bmu_{12}(\x_{12})$ \\\hline
F & 0 & - \\
F & 1 & - \\
M & 0 & - \\
M & 1 & - \\
\multicolumn{3}{c}{} \\
\multicolumn{3}{c}{} \\
\end{tabular}
\caption{$\bmu_{12}$}
\end{subtable}
\hspace{4em}
\begin{subtable}{0.22\textwidth}
\begin{tabular}{cc|c}
\multicolumn{2}{c}{$\x_{13}$} & $\bmu_{13}(\x_{13})$ \\\hline
F & D & - \\
F & R & - \\
F & I & - \\
M & D & - \\
M & R & - \\
M & I & - \\
\end{tabular}
\caption{$\bmu_{13}$}
\end{subtable}
\caption{ marginals on $(1,2)$ and $(1,3)$ from toy dataset in \cref{example:toydata}. \label{table:marginals} }
\end{table*}
\end{example}



\begin{definition}[Graphical model] \label{def:pgm}
  Let $\p_{\btheta}(\x) = \frac{1}{Z} \exp \big(\sum_{C \in \C} \btheta_C(\x_C) \big)$ be a normalized distribution, where $\btheta_C \in \R^{n_C}$. This distribution is a graphical model that factors over the set of cliques $\C$. The vector $\btheta = (\btheta_C)_{C \in \C}$ is the parameter vector.
  \label{def:graphical-model}
\end{definition}

\begin{theorem}[Maximum entropy \cite{wainwright2008graphical}] \label{theorem:maxent}
  Given any $\hat{\bmu}$ in the interior of $\marg$ there is a parameter vector $\hat{\btheta}$ such that the graphical model $\p_{\hat{\btheta}}(\x)$ has maximum entropy among all $\hat{\p}(\x)$
with marginals $\hat{\bmu}$.\footnote{If the marginals are on the boundary of $\marg$, e.g., if they contain zeros, there is a sequence of parameters $\{\btheta^{(n)}\}$ such that $\p_{\btheta^{(n)}}(\x)$ converges to the maximum-entropy distribution as $m \to \infty$. See~\cite{wainwright2008graphical}.}
\end{theorem}

\begin{example}[Graphical Model] \label{example:pgm}
\cref{table:pgm} shows an example graphical model defined over the cliques $\C = \set{(1,2), (1,3)}$. One can easily verify the entries \cref{table:pgm} (b) match the formula stated in \cref{def:pgm}.  For example, for $ \x = \begin{bmatrix} F & 0 & D \end{bmatrix} $, we see that $\p_{\btheta}(\x) = \exp{\big(\btheta_{12}(\x_{12}) + \btheta_{13}(\x_{13}) \big)} = \exp{(123 + 456)} = 789$. (In this case, the normalization constant is $1$) 

\begin{table*}[h] 
\captionsetup[subtable]{position = below}
\captionsetup[table]{position=top}
\begin{subtable}{0.22\textwidth}
\begin{tabular}{cc|c}
\multicolumn{2}{c}{$\x_{12}$} & $\btheta_{12}(\x_{12})$ \\\hline
F & 0 & - \\
F & 1 & - \\
M & 0 & - \\
M & 1 & - \\
\multicolumn{3}{c}{}\\
\multicolumn{2}{c}{$\x_{13}$} & $\btheta_{13}(\x_{13})$ \\\hline
F & D & - \\
F & R & - \\
F & I & - \\
M & D & - \\
M & R & - \\
M & I & - \\
\end{tabular}
\caption{$\btheta_{12}$ and $\btheta_{13}$}
\end{subtable}
\hspace{4em}
\begin{subtable}{0.24\textwidth}
\begin{tabular}{ccc|c}
\multicolumn{3}{c}{$\x$} & $\p_{\btheta}(\x)$ \\\hline
%1 (Gender) & 2 (City) & 3 (Party) & Count \\\hline
F & 0 & D & - \\
F & 0 & R & - \\
F & 0 & I & - \\
F & 1 & D & - \\
F & 1 & R & - \\
F & 1 & I & - \\
M & 0 & D & - \\
M & 0 & R & - \\
M & 0 & I & - \\
M & 1 & D & - \\
M & 1 & R & - \\
M & 1 & I & - \\
%\multicolumn{3}{c}{Total} & 1000 \\
\end{tabular}
\caption{Graphical model, $\p_{\btheta}$}
\end{subtable}
\caption{ TODO \label{table:pgm}}
\end{table*}
\end{example}


\begin{remark}[Efficient Marginal Inference]
In addition to providing a compact factored representation of a high-dimensional data distribution, graphical models enable efficient marginal inference.  Specifically, one can use the well-known belief propagation algorithm to compute $\bmu_{C}$ efficiently from $\btheta$ without every fully materializing $\p_{\btheta}$.  

\end{remark}



==> lessons.tex <==
\section{Lessons Learned}

The following describes the rational for the algorithm design decisions made above, along with lessons learned.

\textbf{Lesson 1.} Knowing the workload (i.e., the evaluation criteria) in advance is essential for designing good mechanisms.  Trying to produce synthetic data that is accurate with respect to all possible downstream tasks will inevitably lead to suboptimal accuracy on the actual downstream tasks that the analyst cares about.  Thus, it is important for the algorithm and/or algorithm designer to be aware of the workload, and use that information implicitly or explicitly.  

The workload used in this competition was particularly challenging due to its enormous size.  Because the 100 random 3-way marginals and 300 random high-order conjunctions were not known ahead of time, they could not be provided as input to the mechanism.  Essentially this meant the algorithm had to be designed to offer accuracy on \emph{all} 3-way marginals and \emph{all} high-order conjunctions.  It would have been interesting to see how the top solutions would have changed if this information was available to the competitors or to the algorithm.  

The third part of the workload, on income inequality and gender wage gap statistics, while more complicated and nonlinear, was actually much easier to handle because it was fixed and known in advance.  Thus, the algorithm could be specifically designed to offer high accuracy on that task.  To accomplish this, it suffices to provide accuracy on the $(Income, Sex, City)$ marginal, which is linear just like the rest of the workload and can be handled in a similar manner.

\textbf{Lesson 2.} Gaussian noise is favorable to Laplace noise in the high-dimensional setting.  The algorithm described in the previous section measures a total of $245$ marginals.  The $L_1$ sensitivty of this function is thus $245$ and the $L_2$ sensitivity is $ \sqrt{245} \approx 15.65 $.  Thus, the scale of Laplace noise required to achieve $(\epsilon, \delta)$-differential privacy is $ \sqrt{2} \cdot 245 / \epsilon \approx 346 / \epsilon $.  The scale of Gaussian noise required can be determined computationally using the moments accountant \cite{abadi2016deep}.  Table \ref{table:noise} compares the magnitude of noise required for each mechanism (in terms of standard deviation).  On average, about $3\times$ less Gaussian noise is required than Laplace noise.  Additionally, the moments accountant is flexible enough to handle \emph{adaptive} composition, which is necessary for the two stages of measurements described above in Step 3 of the algorithm.

\begin{table}[]
\centering
\begin{tabular}{c|cc}
$\epsilon$ & Laplace & Gaussian \\\hline
0.3 & 1155        & 383         \\
1.0 & 346        & 116         \\
8.0 & 43        & 15        
\end{tabular}
\caption{Standard deviation of Laplace and Gaussian noise required to obtain $(\epsilon, \delta)$-differential privacy.} \label{table:noise}
\end{table}

\textbf{Lesson 3.} The domain compression step improved efficiency and utility.  It improved the efficiency of the post-processing step, whose complexity depends on the number of cells in the noisy marginals.  As many of the counts in the one-way marginals were zero or very low, this shrunk the domain quite substantially.  In fact, without this domain compression step, the post-processing would have required orders of magnitude more memory to run.  As $\epsilon$ decreased the domain compression became more aggresive and efficiency improved.  Additionally, by truncating low counts, the algorithm is trading a small amount of bias for a large amount of variance, and consequently improving utility.

\textbf{Lesson 4.} Having access to a provisional (public) dataset greatly simplified algorithm design.  In particular, Step 2 of the algorithm used the provisional data to identify a good set of marginals to measure based on correlations between attributes.  In principle, it is possible to use a differentially private version of that procedure on the true private data, but it is not obvious how to implement that because the sensitivity of mutual information is not easy to reason about and may be high.  It is left as an interesting and important open problem for applying these ideas to settings when provisional data is not available and understanding the impact of provisional data that poorly approximates the final data.

\textbf{Lesson 5.} Selecting the right statistics to measure about the dataset is challenging.  Measuring too many statistics would require adding too much noise to those statistics to satisfy privacy.  On the other hand, with too few statistics, the synthetic data would not be able to capture enough properties of the true data distribution.  Additionally, measurements should only be taken if they improve accuracy on the statistics that matter --- those in the workload.  The mutual information criteria used in the algorithm draws inspiration from similar ideas that have been succesffully applied in the literature \cite{chen2015differentially,zhang2017privbayes}.  Another interesting problem is determining the right way to divide the privacy budget among the measurements.  The algorithm equally divided the budget among the measurements (except for the special case of the (INCOME, SEX, CITY) marginal), but the problem of privacy budget allocation warrants further research.

\textbf{Lesson 6.} Generating synthetic data that matches the measured statistics is a hard problem.  Using recently published ideas, this can be accomplished using graphical models \cite{McKenna19Graphical-model}.  The underlying estimation algorithm is capable of scaling to high-dimensional datasets, but the complexity depends on the structure of the measurements taken in a nuanced way.  In particular, if the graphical model implied by the measured marginals has low tree-width \cite{wainwright2008graphical}, then the estimation algorithm is able to scale.  This insight influenced Step 2 of the algorithm, as the marginals selected are those along the edges of a (maximum spanning) tree.  



==> select_example.tex <==
\newpage
\ryref{
Recall from \cref{sec:eval} that the utility of the synthetic data is judged according to its ability to preserve 3-way marginals, high-order conjunctions, and income inequality statistics.  Thus, measurements should be chosen that will help increase utility according to these metrics.  

Since we need to preserve all 3-way marginals to score well on the first metric, a natural idea would be to measure all 3-way marginals.  However, this is a bad idea for two reasons.  First, since there are a total of $\binom{98}{3}= 152096$ 3-way marginals, it would require an inordinate amount of noise to answer them all, which would result in very poor utility.  Second, even if the privacy budget was large enough where we could answer all 3-way marginals with a reasonable amount of noise, it is actually NP-hard to generate synthetic data that is consistent with those marginals in the worst case\cite{ullman2020pcps}.  

This is not the end of the story, however.  It's often possible to accurately estimate 3-way marginals without measuring them, if the dataset has certain low-dimensional structure common in real-world settings.  \cref{example:3way} demonstrates this idea more concretely.  %we show that some 3-way marginals can be accurately estimated by \pgm even if they are not directly measured.  

\begin{example}[Estimating 3-way marginals] \label{example:3way}
Building on \cref{example:boost,example:estimating}, we show two 2-way marginals (with no noise) in Table (a).  Plugging these into \pgm, we can find the maximum entropy 3-way marginal that is consistent with those 2-way marginals, which we show in Table (b).  This is pretty close to the true 3-way marginal, shown in Table (c).  In fact, the normalized $L_1$ error is only $\approx 0.09$, which is quite good.  Thus, there are some cases where we can estimate 3-way marginals reasonably well using only 2-way marginals.  In this case, it worked well because \attr{SEX} and \attr{SCHOOL} are (approximately) conditionally independent given \attr{LABFORCE}.  
\begin{table*}[h]
\hspace{-2em}
\captionsetup[subtable]{position = below}
\captionsetup[table]{position=top}
\begin{adjustbox}{width=0.91\textwidth}
\begin{subtable}{0.3\textwidth}
\begin{tabular}{cc|r}
\hline
\texttt{SEX} & \texttt{LABFORCE} & \multicolumn{1}{c}{\emph{count}} \\\hline
M & --- & $156$ \\
M & N & $65$ \\
M & Y & $316$ \\
F & --- & $158$ \\
F & N & $282$ \\
F & Y & $23$ \\\hline\hline
\texttt{LABFORCE} & \texttt{SCHOOL} & \multicolumn{1}{c}{\emph{count}} \\\hline
--- & N & $159$ \\
--- & Y & $155$ \\
N & N & $288$ \\
N & Y & $59$ \\
Y & N & $336$ \\
Y & Y & $3$ \\\hline
\end{tabular}
\caption{2-way marginals}
\end{subtable}
\hspace{2em}
\begin{subtable}{0.3\textwidth}
\begin{tabular}{ccc|r}
\hline
\texttt{SEX} & \texttt{LABFORCE} & \attr{SCHOOL} & \multicolumn{1}{c}{\emph{count}} \\\hline
M & --- & N & $78.994$ \\
M & --- & Y & $77.006$ \\
M & N   & N & $53.948$ \\
M & N   & Y & $11.052$ \\
M & Y   & N & $313.204$ \\
M & Y   & Y & $2.796$ \\
F & --- & N & $80.006$ \\
F & --- & Y & $77.994$ \\
F & N   & N & $234.052$ \\
F & N   & Y & $47.948$ \\
F & Y   & N & $22.796$ \\
F & Y   & Y & $0.204$ \\
\multicolumn{4}{c}{}
\end{tabular}
\caption{\pgm estimate}
\end{subtable}
\hspace{4em}
\begin{subtable}{0.3\textwidth}
\begin{tabular}{ccc|r}
\hline
\texttt{SEX} & \texttt{LABFORCE} & \attr{SCHOOL} & \multicolumn{1}{c}{\emph{count}} \\\hline
M & --- & N & $74$ \\
M & --- & Y & $82$ \\
M & N   & N & $36$ \\
M & N   & Y & $29$ \\
M & Y   & N & $313$ \\
M & Y   & Y & $3$ \\
F & --- & N & $85$ \\
F & --- & Y & $73$ \\
F & N   & N & $252$ \\
F & N   & Y & $30$ \\
F & Y   & N & $23$ \\
F & Y   & Y & $0$ \\
\multicolumn{4}{c}{}
\end{tabular}
\caption{3-way marginal}
\end{subtable}
\end{adjustbox}
\end{table*}
\end{example}

In general, if the dataset satisfies conditional independence assumptions of the form shown in \cref{example:3way}, then measuring a small set of 2-way marginals can lead to quite accurate estimates of 3-way marginals.  To determine which 2-way marginals should be measured, note that it is not neccessary to measure ones where the corresponding attributes are statistically independent (or approximately so), as we can already estimate them well just using the one-way marginals that we measure anyway.  Therefore, \mech selects 2-way marginals by looking at the \emph{mutual information} between attributes, and selecting pairs of attributes that are highly correlated according to this measure.  However, it is not as simple as just selecting the top $k$ most correlated attribute pairs.  In order for \pgm to run efficiently, the graphical model that results from the chosen attribute pairs needs to be approximatley tree like.  For that reason, \mech identifies the maximum spanning tree of the complete graph, where nodes correspond to attributes, and edges measure mutual information between attributes.  This ensures that \pgm will run efficiently, while also selecting highly correlated attribute pairs.  A reader familiar with graphical models will recognize this as the celebrated Chow and Liu algorithm for structure learning in a graphical model.}{not sure what to do with this}


==> table_3col.tex <==
\begin{table}
\begin{tabular}{ll|ll|ll}
\midrule
SPLIT     &         2/2 & CLASSWKR  &        10/4 & MIGSEA5   &     998/510 \\
SPANNAME  &         3/4 & INCNONWG  &        10/4 & IND1950   &     998/162 \\
VETWWI    &         3/3 & SAMEPLAC  &        10/4 & OCC       &     999/231 \\
LABFORCE  &         3/3 & MARRNO    &       10/10 & MIGPLAC5  &    1000/199 \\
SCHOOL    &         3/2 & VETSTAT   &        10/4 & UIND      &    1000/136 \\
SEX       &         3/2 & OWNERSHPD &        21/8 & EDUCD     &     1000/44 \\
RESPONDT  &         3/3 & FAMSIZE   &       22/29 & UOCC      &    1000/231 \\
SLREC     &         3/2 & SIZEPL    &       31/19 & GQTYPED   &     1000/92 \\
OWNERSHP  &         3/3 & EMPSTATD  &       35/15 & DURUNEMP  &      1000/- \\
FARM      &         3/3 & WKSWORK1  &       53/53 & IND       &    1000/136 \\
SSENROLL  &         3/3 & SEA       &        54/- & OCC1950   &    1000/283 \\
URBAN     &         3/3 & OCCSCORE  &       81/81 & HIGRADED  &     1000/69 \\
METRO     &         4/5 & AGEMARR   &       90/89 & UOCC95    &    1000/279 \\
EMPSTAT   &         4/4 & MIGRATE5D &       91/15 & COUNTY    &    1251/385 \\
HISPAN    &         5/6 & MTONGUE   &       97/92 & ENUMDIST  &      3021/- \\
CITIZEN   &         5/6 & SEI       &       97/97 & URBPOP    &      3225/- \\
WARD      &         6/- & HRSWORK1  &       99/99 & CITYPOP   &      3225/- \\
NATIVITY  &         6/6 & CLASSWKRD &       99/18 & METAREAD  &    6561/378 \\
WKSWORK2  &         7/7 & GQFUNDS   &      100/13 & MTONGUED  &    9602/489 \\
RACE      &         7/9 & EDUC      &      100/13 & NPBOSS50  &  10000/1002 \\
MARST     &         7/6 & CHBORN    &      100/62 & RENT      &     10000/- \\
NCHLT5    &        7/10 & HIGRADE   &      100/25 & MIGCOUNTY &   10000/385 \\
GQ        &         7/7 & AGEMONTH  &      100/15 & CITY      &  10000/1164 \\
VET1940   &         9/4 & VETSTATD  &      100/10 & MIGCITY5  &  10000/1164 \\
VETPER    &         9/8 & AGE       &     109/130 & ERSCOR50  &  10000/1002 \\
HISPRULE  &         9/9 & HISPAND   &      481/55 & EDSCOR50  &  10000/1002 \\
UCLASSWK  &         9/8 & RACED     &     621/238 & MIGMET5   &   10000/379 \\
HRSWORK2  &         9/9 & SUPDIST   &       631/- & MBPLD     &   90021/537 \\
GQTYPE    &       10/10 & METAREA   &     657/334 & FBPLD     &   90021/539 \\
VETCHILD  &        10/5 & PRESGL    &       816/- & BPLD      &   90022/536 \\
MIGRATE5  &        10/7 & MBPL      &     901/164 & INCWAGE   &    999999/- \\
MIGTYPE5  &        10/6 & FBPL      &     901/165 & VALUEH    &  10000000/- \\
SAMESEA5  &        10/6 & BPL       &     901/163 & & \\
\bottomrule
\end{tabular}
\caption{ \label{table:domain} Domain information for the census dataset used in the third round of the competition.  Table specifies both column names, and number of possible values for that column from two different sources: (1) the provided ``specs'' file and (2) the IPUMS documentation}
\end{table}

\ry{label rows/cols}


==> table_4col.tex <==
\begin{table}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{ll|ll|ll|ll}
\midrule
1. \attr{SPLIT} & 2/2 & 26. \attr{VETPER} & 9/8 & 51. \attr{HRSWORK1} & 99/99 & 76. \attr{UOCC} & 1000/231 \\
2. \attr{SLREC} & 3/2 & 27. \attr{HISPRULE} & 9/9 & 52. \attr{VETSTATD} & 100/10 & 77. \attr{UOCC95} & 1000/279 \\
3. \attr{SEX} & 3/2 & 28. \attr{HRSWORK2} & 9/9 & 53. \attr{GQFUNDS} & 100/13 & 78. \attr{OCC1950} & 1000/283 \\
4. \attr{SCHOOL} & 3/2 & 29. \attr{CLASSWKR} & 10/4 & 54. \attr{EDUC} & 100/13 & 79. \attr{DURUNEMP} & 1000/1000 \\
5. \attr{URBAN} & 3/3 & 30. \attr{INCNONWG} & 10/4 & 55. \attr{AGEMONTH} & 100/15 & 80. \attr{COUNTY} & 1251/385 \\
6. \attr{FARM} & 3/3 & 31. \attr{SAMEPLAC} & 10/4 & 56. \attr{HIGRADE} & 100/25 & 81. \attr{ENUMDIST} & 3021/3021 \\
7. \attr{OWNERSHP} & 3/3 & 32. \attr{VETSTAT} & 10/4 & 57. \attr{CHBORN} & 100/62 & 82. \attr{CITYPOP} & 3225/3225 \\
8. \attr{RESPONDT} & 3/3 & 33. \attr{VETCHILD} & 10/5 & 58. \attr{AGE} & 109/109 & 83. \attr{URBPOP} & 3225/3225 \\
9. \attr{SPANNAME} & 3/3 & 34. \attr{MIGTYPE5} & 10/6 & 59. \attr{HISPAND} & 481/55 & 84. \attr{METAREAD} & 6561/378 \\
10. \attr{LABFORCE} & 3/3 & 35. \attr{SAMESEA5} & 10/6 & 60. \attr{RACED} & 621/238 & 85. \attr{MTONGUED} & 9602/489 \\
11. \attr{VETWWI} & 3/3 & 36. \attr{MIGRATE5} & 10/7 & 61. \attr{SUPDIST} & 631/631 & 86. \attr{MIGMET5} & 10000/379 \\
12. \attr{SSENROLL} & 3/3 & 37. \attr{GQTYPE} & 10/10 & 62. \attr{METAREA} & 657/334 & 87. \attr{MIGCOUNTY} & 10000/385 \\
13. \attr{METRO} & 4/4 & 38. \attr{MARRNO} & 10/10 & 63. \attr{PRESGL} & 816/816 & 88. \attr{ERSCOR50} & 10000/1002 \\
14. \attr{EMPSTAT} & 4/4 & 39. \attr{OWNERSHPD} & 21/8 & 64. \attr{BPL} & 901/163 & 89. \attr{EDSCOR50} & 10000/1002 \\
15. \attr{HISPAN} & 5/5 & 40. \attr{FAMSIZE} & 22/22 & 65. \attr{MBPL} & 901/164 & 90. \attr{NPBOSS50} & 10000/1002 \\
16. \attr{CITIZEN} & 5/5 & 41. \attr{SIZEPL} & 31/19 & 66. \attr{FBPL} & 901/165 & 91. \attr{CITY} & 10000/1164 \\
17. \attr{WARD} & 6/6 & 42. \attr{EMPSTATD} & 35/15 & 67. \attr{IND1950} & 998/162 & 92. \attr{MIGCITY5} & 10000/1164 \\
18. \attr{NATIVITY} & 6/6 & 43. \attr{WKSWORK1} & 53/53 & 68. \attr{MIGSEA5} & 998/510 & 93. \attr{RENT} & 10000/10000 \\
19. \attr{MARST} & 7/6 & 44. \attr{SEA} & 54/54 & 69. \attr{OCC} & 999/231 & 94. \attr{MBPLD} & 90021/537 \\
20. \attr{GQ} & 7/7 & 45. \attr{OCCSCORE} & 81/81 & 70. \attr{EDUCD} & 1000/44 & 95. \attr{FBPLD} & 90021/539 \\
21. \attr{NCHLT5} & 7/7 & 46. \attr{AGEMARR} & 90/89 & 71. \attr{HIGRADED} & 1000/69 & 96. \attr{BPLD} & 90022/536 \\
22. \attr{RACE} & 7/7 & 47. \attr{MIGRATE5D} & 91/15 & 72. \attr{GQTYPED} & 1000/92 & 97. \attr{VALUEH} & 10000000/5003 \\
23. \attr{WKSWORK2} & 7/7 & 48. \attr{MTONGUE} & 97/92 & 73. \attr{IND} & 1000/136 & 98. \INCWAGEA & ---/52 \\
24. \attr{VET1940} & 9/4 & 49. \attr{SEI} & 97/97 & 74. \attr{UIND} & 1000/136 & 99. \INCWAGEB & ---/8 \\
25. \attr{UCLASSWK} & 9/8 & 50. \attr{CLASSWKRD} & 99/18 & 75. \attr{MIGPLAC5} & 1000/199 & \quad\:\: \attr{INCWAGE} & 10000000/--- \\
\bottomrule
\end{tabular}%
}
\caption{ \label{table:domain} Domain information for the census dataset used in the third round of the competition.  Table specifies both attribute names, and number of possible values for that attribute according to (1) the provided specs file and (2) the specs file combined with IPUMS documentation.}
\end{table}

